ReverseORC: Reverse Engineering of Resizable User Interface Layouts with OR-Constraints

Reverse engineering (RE) of user interfaces (UIs) plays an important role in software evolution. However, the large diversity of UI technologies and the need for UIs to be resizable make this challenging. We propose ReverseORC, a novel RE approach able to discover diverse layout types and their dynamic resizing behaviours independently of their implementation, and to specify them by using OR constraints. Unlike previous RE approaches, ReverseORC infers flexible layout constraint specifications by sampling UIs at different sizes and analyzing the differences between them. It can create specifications that replicate even some non-standard layout managers with complex dynamic layout behaviours. We demonstrate that ReverseORC works across different platforms with very different layout approaches, e.g., for GUIs as well as for the Web. Furthermore, it can be used to detect and fix problems in legacy UIs, extend UIs with enhanced layout behaviours, and support the creation of flexible UI layouts.

==> 12-Removed-Part.tex <==
\begin{DELETE}
\section{Topological Equivalence of layouts}
    
One important step in detecting layout behaviors and differences is to check whether two layouts $L1$ and $L2$ are topologically equivalent. It is a challenging task since topological equivalence cannot rely on direct comparisons of widget sizes and positions in the layouts. Even if all the widgets have different sizes and positions in the two layouts $L1$ and $L2$, they can still be topologically equivalent. In our approach, we use widget alignments to check topological equivalence.

\subsection{Widget Mapping}

 \begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
\SetAlgoLined
\begin{DELETE}
\SetKwProg{Fn}{Function}{}{end}
\Fn{\textit{WidgetMapping}(L1, L2)}{

    $\textit{widgetMap} \leftarrow \{\}$
    
    $\textit{L1ResidualWidgets} \leftarrow L1.\textit{Widgets}$
    
    $\textit{L2ResidualWidgets} \leftarrow L2.\textit{Widgets}$
    
    \For{$w1 \in L1.\textit{Widgets}$} {
        
        \If  {($\exists \ w2 \in \textit{L2ResidualWidgets}$ such that $w1.id  ==  w2.id$)} {
            
            $\textit{widgetMap} \leftarrow \textit{widgetMap} \ \cup \ \{w1 \mapsto w2\}$
            
            $\textit{L1ResidualWidgets}.remove(w1)$
            
            $\textit{L2ResidualWidgets}.remove(w2)$
        }
    }
    \Return $\textit{widgetMap}$, $\textit{L1ResidualWidgets}$, $\textit{L2ResidualWidgets}$
}
\end{DELETE}
 
\caption{Widget Mapping Creation}
\label{alg:widgetMapping}
\end{algorithm}


We first create a widget mapping $\textit{widgetMap}$ between the two layouts $L1$ and $L2$ based on the unique widget ids (Algorithm \ref{alg:widgetMapping}), which are typically shared between the two layouts.Initially, we set $\textit{widgetMap}$ to be an empty mapping (Line 1). Line 2 and 3 create two sets of widgets to keep track of the widgets that have not yet been mapped in $\textit{widgetMap}$. 

Lines 5-11 indicate how we add new element to $\textit{widgetMap}$. For each widget $w1$ in the layout $L1$, we check whether there is a corresponding widget $w2$ in the layout $L2$ such that $w1$ and $w2$ have the same widget identity (Line 6). If so, based on $w1$ to $w2$ (Line 7) we add a new element to $\textit{widgetMap}$ and remove $w1$ and $w2$ from the respective widget lists (Line 8-9). In the end, we get a widget mapping $\textit{widgetMap}$ between the corresponding widgets in the two layouts and two lists of widgets that do not appear in the respective other layout (Line 12).


\subsection{Tabstop Mapping}

 \begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
\SetAlgoLined
\begin{DELETE}

\SetKwProg{Fn}{Function}{}{end}
\Fn{TabstopMap(\textit{widgetMap}, xtabs, ytabs)} {

    $\textit{tabMap} \leftarrow \{\}$
    
    $mismatchedXTabs \leftarrow \{\}$
    
    $mismatchedYTabs \leftarrow \{\}$

    $residualXTabs \leftarrow set(Image(xtabs))$
    
    $residualYTabs \leftarrow set(Image(ytabs))$
    
    \For {$w1 \in Domain(\textit{widgetMap})$} {
    
        $w2 \leftarrow \textit{widgetMap}[w1]$
        
        \If {$\textit{tabMap}[w1.\textit{leftTab}] == NULL$} {
            $tabMap[w1.\textit{leftTab}] \leftarrow w2.\textit{\textit{leftTab}}$

            $residualXTabs.remove(w2.\textit{leftTab})$ 
        } \Else {
            \If {$\textit{tabMap}[w1.\textit{leftTab}] \neq w2.\textit{leftTab}$} {
                $\textit{mismatchedXTabs} \leftarrow \textit{mismatchedXTabs} \ \cup\ \{w2.\textit{leftTab} \rightarrow \textit{tabMap}[w1.\textit{leftTab}]\}$
            }
        }

        Process right, top, bottom tabstops analogously.
        
        % \If {$tabMap[w1.rightTab] == NULL$} {
        %     $tabMap[w1.rightTab] \leftarrow w2.rightTab$
            
        %     $residualXTabs.remove(w2.rightTab)$
        %     } \Else {
        %     \If {$tabMap[w1.rightTab] \neq w2.rightTab$} {
        %         $mismatchedXTabs \leftarrow mismatchedXTabs \ \cup\ \{w2.rightTab\}$
        %     }
        % }
        
        % \If {$tabMap[w1.topTab] == NULL$} {
        %     $tabMap[w1.topTab] \leftarrow w2.topTab$
            
        %     $residualYTabs.remove(w2.topTab)$
        %     } \Else {
        %     \If {$tabMap[w1.topTab] \neq w2.topTab$} {
        %         $mismatchedYTabs \leftarrow mismatchedYTabs \ \cup\ \{w2.topTab\}$
        %     }
        % }
        
        % \If {$tabMap[w1.bottomTab] == NULL$} {
        %     $tabMap[w1.bottomTab] \leftarrow w2.bottomTab$
            
        %     $residualYTabs.remove(w2.bottomTab)$
        %     } \Else {
        %     \If {$tabMap[w1.bottomTab] \neq w2.bottomTab$} {
        %         $mismatchedYTabs \leftarrow mismatchedYTabs \ \cup\ \{w2.bottomTab, \}$
        %     }
        % }
    }
    \Return $\textit{mismatchedXTabs}$, $\textit{mismatchedYTabs}$, $residualXTabs$, $residualYTabs$
 }
 \end{DELETE}
 

\caption{Tabstop Map Creation}
\label{alg:tabstopmappingcreation}
\end{algorithm}

Based on the results from the tabstop creation, we construct a tabstop mapping as a hash table $tabMap$, which maps from tabstops in one layout $L1$ to tabstops in another layout $L2$ and which also keeps track of the differences of tabstops in the two layouts (Algorithm \ref{alg:tabstopmappingcreation}). The tabstop mapping hash table $tabMap$ is empty initially (Line 2).

When we add mappings for the layout $L2$ to the hash table, we also keep track of the set of mismatched tabstops and the set of residual tabstops. We create a hash table for each set of mismatched tabstops ($mismatchedXtabs$, $mismatchedYtabs$). Whenever a tabstop has a conflict for mapping from its corresponding tabstop in $L1$, we add a mapping from it to the tabstop it conflicts with to the hash table. The sets of residual tabstops ($residualXtabs$, $residualYtabs$) contain all the tabstops that have not been mapped from tabstops in $L1$. Initially, mismatched tabstop hash tables are empty (Line 3-4) and residual tabstop sets contain all the tabstops in the layout $L2$ (Line 5-6). 

We loop over all the widgets in the domain of the $\textit{widgetMap}$ generated by the Algorithm~\ref{alg:widgetMapping}, since these widgets are the ones in the layout $L1$ that have corresponding widgets in the other layout $L2$ (Line 7). For each widget $w1$ in the loop, we use $\textit{widgetMap}$ to get its corresponding widget $w2$ in the layout $L2$ (Line 8). Ideally, the four tabstops of $w1$ should correspond to the four tabstops of $w1$. In the ideal case, if $w1.\textit{leftTab}$ has already mapped to $w2.\textit{leftTab}$ in the tabstop mapping hash table $tabMap$ and we do not need to do anything. If $w1.\textit{leftTab}$ has not been mapped to any tabstop, then we add an element to $tabMap$ mapping from $w1.\textit{leftTab}$ to $w2.\textit{leftTab}$. We then remove $w2.\textit{leftTab}$ from $residualXtabs$ as $w2.\textit{leftTab}$ has been mapped from a $L1$ tabstop $w1.\textit{leftTab}$ (Line 9-12). Otherwise, if $w1.\textit{leftTab}$ has already been mapped to a tabstop in the layout $L2$ but it is not the same tabstop variable as $w2.\textit{leftTab}$, it causes a conflict since one tabstop in the layout $L1$ would be mapped to two different tabstops in the layout $L2$. Then we record this conflict by adding the mapping from $w2.\textit{leftTab}$ to $w1.\textit{leftTab}$ to the hash map of mismatched tabstops (Line 14-16). 

Through this algorithm, we get a tabstop map hash table mapping from tabstops in the layout $L1$ to tabstops in the layout $L2$, two hash tables of mismatched tabstops in $L2$ containing conflicting tabstops, and two sets of residual tabstops containing tabstops that cannot be mapped into the other one.


% \DELETE{\subsection{Topological Equivalence Check}}
\subsection{Topological Equivalence Check}

 \begin{algorithm}[t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
\SetAlgoLined
\begin{DELETE}
\SetKwProg{Fn}{Function}{}{end}
\Fn{\textit{TopologicalEquivalenceCheck}(L1, L2)} {
    
    $\textit{widgetMap}$, $\textit{L1ResidualWidgets}$, $\textit{L2ResidualWidgets}$ $\leftarrow$ $\textit{WidgetMapping}(L1,\ L2)$
    
    \If {($\textit{L1ResidualWidgets} \neq  \emptyset$ OR $\textit{L2ResidualWidgets} \neq  \emptyset$)} {
        \Return $FALSE$
    }
    
    $xtabs1$, $ytabs1 = \textit{TabstopCreation}(L1)$
    
    $xtabs2$, $ytabs2 = \textit{TabstopCreation}(L2)$
    
    $L2MismatchedXTabs$, $L2MismatchedYTabs$, $L2ResidualXTabs$, $L2ResidualYTabs \leftarrow \textit{TabstopMapping}(\textit{widgetMap}$, $xtabs2$, $ytabs2)$
    
    $L1MismatchedXTabs$, $L1MismatchedYTabs$, $L1ResidualXTabs$, $L1ResidualYTabs \leftarrow \textit{TabstopMapping}(\textit{widgetMap}^{-1})$, $xtabs1$, $ytabs1)$
    
    $\textit{L1DiffXTabs} \leftarrow L1MismatchedXTabs.keys() - L1ResidualXTabs$
    
    $\textit{L1DiffXTabs} \leftarrow \textit{L1DiffXTabs} \ \cup \ \{L1MismatchedXTabs[tab]$ for each $\textit{tab}$ in $\textit{L1DiffTabs}$
    
    Compute $\textit{L1DiffYTabs}$, $\textit{L2DiffXTabs}$, and $\textit{L2DiffYTabs}$ analogously.
    
    \If {$(len(\textit{L1DiffXTabs}) == 0)$ AND $(len(\textit{L1DiffYTabs}) == 0)$ AND $(len(\textit{L2DiffXTabs}) == 0)$ AND $(len(\textit{L2DiffYTabs}) == 0)$} {
        \Return $TRUE$
    } \Else {
        \Return $FALSE$
    }
 }
 \end{DELETE}

\caption{Topological Equivalence Check}
\label{alg:topologicalequivalencecheck}
\end{algorithm}


Two layouts $L1$ and $L2$ are topologically equivalent if and only if both the widgets and the tabstops in them are equivalent (Algorithm \ref{alg:topologicalequivalencecheck}). 

The equivalence of the widgets in two layouts requires that each widget in one layout has a corresponding widget with the same widget identity in the other layout, and vice versa. As $\textit{WidgetMapping}$ is a function mapping all the widgets with the same widget identifiers in the two layouts and also returns two respective sets of the widgets in the two layouts that do not have a corresponding widgets in the other layout. Thus, we can simply check whether these two sets are empty. If any one of them are not empty, it means that some widget does not have corresponding widget in the other layout, so that the widgets in the two layouts are not equivalent (Line 2-5).

Line 6-9 create tabstops for both layouts and construct tabstop mappings from the tabstops in $L1$ to the tabstops in $L2$ and vice versa. Note that $widgetMap^{-1}$ in Line 9 is the inverse mapping of $\textit{widgetMap}$. It maps from the widgets in the layout $L2$ to their corresponding widgets in the layout $L1$. Thus, $TabstopMap(widgetMap^{-1})$ maps from the tabstops in $L2$ to the tabstops in $L1$. Note that the tabstop mapping from $L2$ to $L1$ is not a valid inverse mapping of the tabstop mapping from $L1$ to $L2$. Consider the case that each tabstop in $L1$ can be mapped to a tabstop in $L2$ but there are more tabstops in $L2$ than in $L1$. Then if we map tabstops from $L2$ to $L1$, some tabstops in the mapping domain cannot be mapped to any tabstop in $L1$.

Theoretically, if two layouts are topologically equivalent and all the tabstops are aligned perfectly, then each tabstop in one layout can be matched to its corresponding tabstop in the other layout. Thus, all the residual tabstop sets and the mismatched tabstop sets should be empty. However, in practice, it is common that widgets could be accidentally aligned or for instance, two touching widgets in one layout move a little bit further away from each other in the other layout. These cases can cause multiple tabstops to be a single tabstop in one layout and lead to some false negative results when checking for tabstop equivalence. 

% \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{figures/equivalent.png}
% \caption{Two layouts L1 and L2 are toplogically equivalent although the sizes and alignments of the widgets are different}
% \label{fig:equivalent}
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{figures/not_equivalent.png}
% \caption{Two layouts L1 and L2 are not toplogically equivalent.}
% \label{fig:not_equivalent}
% \end{figure}

To address this problem, we check whether the mismatched tabstops are the same as the residual tabstops since if it is the case, then it means all the mismatched tabstops are caused by accidentally alignments. The intuition behind this is that any misalignment that changes the topology will increase the number of mismatched tabstops, while the number of residual tabstops will remain the same. However, if it is a accidental misalignment, then the mismatched tabstop will also be a residual tabstop. If two widgets are aligned accidentally in one layout $L1$ and not aligned in the other layout $L2$, then for these two widgets, there is one more, additional tabstop in $L2$ than in $L1$. This yields a conflict in that one tabstop in $L1$ can be mapped to two different tabstops in $L2$, one of which causes the conflict. If the tabstop that causes the conflict is not mapped from another tabstop in $L1$, then it is both a mismatched and a residual tabstop. For example, in Figure~\ref{fig:equivalent}, the tabstop $x1$ in the layout $L1$ is mapped to both $a1$ and $a2$ in $L2$. According to our algorithm, when we process the Widget 3, we add $a2$ to the mismatched tabstop set. However, as no other tabstop in $L1$ maps to $a2$, $a2$ is also in the residual tabstop set. On the other hand, if a widget breaks the topological equivalence, for example, in a flow layout, a widget moves from the end of the previous row to the beginning of the next row. The left tabstop of the moved widget is the same as the left boundary of the flow layout which is already a defined tabstop. When we construct tabstop mappings between the two layouts, the left tabstop of this widget is an mismatched tabstop but not a residual tabstop as it is also mapped by some other widget's tabstop. As shown in Figure~\ref{fig:not_equivalent}, $y1$ in $L1$ is mapped to both $b1$ as we process Widget 1 and $b2$ as we process Widget 4 in $L2$, which causes a conflict, but $b2$ is also mapped from $y2$ in the layout $L1$. In this case, mismatched tabstops are not identical to residual tabstops, as $b2$ is a mismatched tabstop but not a residual one, and thus the two layouts are not topological equivalent. 

To check whether mismatched tabstops are the same as residual tabstops and further identify the difference, we compute the difference between the keys of the mismatched tabstop hash tables, which are the tabstops causing conflicts and the set of residual tabstops (Line 10). This resulting set highly depends on the order in which we process the tabstops, as when two tabstops conflicts with each other, the conflict cannot be found when we process the first one, and only processing the second one will identify the conflict. However, the conflict is caused by both tabstops. The hash table of mismatched tabstops contains the mappings from the tabstop causing the conflict to the one it conflicts with. Thus, we finally also add the tabstop that each one in the difference set conflicts with to the difference set (Line 11). In the end, if all the difference sets are empty, then the tabstops in the two layouts are topologically equivalent.



\begin{table*}[h!]
  \centering
  \begin{DELETE}
 \begin{tabular}{ | p{0.475\textwidth} | p{0.475\textwidth} |}
    \hline
    \multicolumn{1}{|c|}{Primitive ORC Layout Pattern}  & \multicolumn{1}{|c|}{Pattern Detection Steps}  \\ \hline
    % \begin{minipage}{0.475\textwidth}
    % \vspace{5mm}
    % \centerline{{\bf Horizontal Flow}}
    % % \vspace{1mm}
    %   \includegraphics[width=\textwidth]{figures/horizontal_flow.png}
    % \end{minipage}
     \vspace{3mm}
    &
    \begin{minipage}{0.475\textwidth}

{
\vspace{1mm}
Detection for horizontal flow in the top toolbar:
   \begin{enumerate}
   \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}
  \item Check whether both residual widget lists from Algorithm~\ref{alg:widgetMapping} are empty. If not, return $False$.
	\item For L1, find the topmost tabstop $\textit{topmostTab}$ in $\textit{L1DiffXTabs}$ and the leftmost tabstop $\textit{leftmostTab}$ in $\textit{L1DiffYTabs}$ (both lists from Algorithm~\ref{alg:topologicalequivalencecheck}). 
	\item For each widget $w$ whose left tabstop is $\textit{leftmostTab}$, check whether its top tabstop $w.topTab$ is either in $\textit{L1DiffXTabs}$ or can be mapped from a tabstop in $\textit{L2DiffXTabs}$ by the tabMap from $L2$ to $L1$ from Algorithm~\ref{alg:tabstopmappingcreation}. If not, return $False$. We put all these $\textit{w.topTab}$s into a list $\textit{L1FlowTopTab}$.
	\item Get all the widgets whose top tabstops are in $\textit{L1FlowTopTabs}$, through the mapping from tabstops to widgets. We call this list of widgets $\textit{L1FlowWidgets}$.
	\item Process the layout $L2$ analogously to get the list $\textit{L2FlowWidgets}$.
	\item Set $\textit{flowWidgets} \leftarrow \textit{L1FlowWidgets}\ \cap \textit{L2FlowWidgets}$. Here widgets are consider identical if they correspond in the two layouts (with identical widget id). 
	\item Remove all the tabstops corresponding to widgets in $flowWidgets$ from $\textit{L1DiffXTabs}$, $\textit{L1DiffYTabs}$, $\textit{L2DiffXTabs}$, $\textit{L2DiffYTabs}$. If all these 4 lists become empty, then return $True$; otherwise, return $False$.
	
\end{enumerate}
}

    \end{minipage}
   
    \\ \hline
    
    % \begin{minipage}{0.475\textwidth}
    % \vspace{5mm}
    % \centerline{{\bf Vertical Flow}}
    % % \vspace{1mm}
    %   \includegraphics[width=\textwidth]{figures/vertical_flow.png}
    % \end{minipage}
     \vspace{3mm}
    &
    \begin{minipage}{0.475\textwidth}

{
\vspace{1mm}
Detection for vertical flow in the left toolbar:

  Analogous computation as for a horizontal flow, but swapping top and left tabstops.
	
}

    \end{minipage}
   
    \\ \hline
    
    
    %  \begin{minipage}{0.475\textwidth}
    % \vspace{5mm}
    % \centerline{{\bf Optional Widget}}
    % % \vspace{1mm}
    %   \includegraphics[width=\textwidth]{figures/optional_widget.png}
    % \end{minipage}
     \vspace{3mm}
    &
    \begin{minipage}{0.475\textwidth}

{
\vspace{1mm}
Detection for one optional widget in the top toolbar:

Return $True$ if

  \begin{enumerate}
   \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}
  \item  $\textit{L1DiffXTabs}$, $\textit{L1DiffYTabs}$, $\textit{L2DiffXTabs}$ and $\textit{L2DiffYTabs}$ in Algorithm~\ref{alg:topologicalequivalencecheck} are all empty.
  \item One of $\textit{L1ResidualWidgets}$ and $\textit{L2ResidualWidgets}$ in Algorithm~\ref{alg:widgetMapping} is empty and the other contains exactly one widget.
\end{enumerate}
}

    \end{minipage}
   
    \\ \hline

  \end{tabular}

  \caption{Detection of primitive ORC layout patterns}\label{tbl:detection}
    \end{DELETE}
\end{table*}

\begin{DELETE}
If two layouts are not topological equivalent, then some nonlinear behaviors exist between these two layouts. To detect nonlinear behaviors, we infer layout types by matching primitive ORC layout patterns based on differences between layout exemplars. We define a set of primitive ORC patterns (Table~\ref{tbl:detection}).
\end{DELETE}

% Note: Many layout behaviors can be used to identify layout patterns. For example, if one item vanishes, then it is an optional item. We can also infer the relative weight and thus relative priority of each optional item based on the order of their disappearance; if an item moves to the next row or the next column, then it is probably in a flow sub-layout; if an item is pivoted around, it may be defined to have alternative positions. We should be able to identify whether a widget has a constant size or a variable size by comparing the widget size in different exemplars. We may also want to detect the existence of grid-bag layout and figure out the relative weights in grid-bag layout. The alignments among widgets can also be used to infer the presence of constraints. if we have 2 layouts and one is wide and one is narrow and in the first one the toolbar is all at the top and then in the second one the toolbar suddenly at the left side and we need to use an appropriate pattern for that.If in the first layout the toolbar is stretched only over one row and then in the second novel layout, it stretches over two rows and it could be some kind of flow layout. We can get the grouping in the accessibility.




\begin{DELETE}
 \subsection{Search Process}
 
%  \begin{figure*}[h!]
% \centering
% \includegraphics[width=\textwidth]{figures/example.pdf}
% \caption{An example to demonstrate the grid search process.}
% \label{fig:example}
% \end{figure*}
 
After each subsampling step, we check for topological equivalence between each newly sampled layout exemplar and its parents. If any checked parent-child pair of layout exemplars are topologically equivalent or match a primitive ORC pattern, then we stop subsampling between this pair. Otherwise, we recursively subsample based on the subsampling rules. 
%We then iteratively update the ORC specification to match the observed layout behaviors and layout patterns. 
 
Whenever a parent-child pair matches a primitive ORC pattern, we add this information to the list of detected primitive ORC patterns. Later checks first ignore the differences caused by already detected primitive ORC patterns. We maintain a list of parent-child pairs that are not topologically equivalent and could not be matched to any primitive ORC layout patterns. After checking all the already sampled pairs, we pop one pair from the list to recheck. If the pair of layouts is still not topologically equivalent or matches a primitive ORC pattern (ignoring all already detected patterns), we subsample this pair. Otherwise, we pop another pair and repeat this process until the list becomes empty. Note that to reduce computation, we prefer to first pick the pairs that subsample only a single new exemplar (b, c in Figure~\ref{fig:sample}) over three new exemplars (a in Figure~\ref{fig:sample}).

% Whenever a new primitive pattern is detected, we recheck all the pairs in the list. If any pair becomes topologically equivalent or matches a primitive pattern by ignoring all the detected patterns, we remove this pair from the list. After we have checked all the already sampled pairs, we subsample a pair in the list, remove it from the list, and repeat the process. We iteratively subsample pairs and perform checks in the list until the list becomes empty.

Here we demonstrate how the search process works through an example. We start with layouts $L1$ and $L2$ sized to the largest and smallest possible window size for the GUI on a given screen.

\begin{enumerate}
    \item ($L1$, $L2$): No match.
    \item Subsample ($L1$, $L2$) to get $L3$, $L4$, $L5$ (Figure~\ref{fig:example} a), then we start comparing each subsampled exemplar with its parents.
    \item ($L1$, $L3$): No match.
    \item ($L1$, $L4$): Left toolbar matches the vertical flow primitive ORC pattern.
    \item ($L1$, $L5$): No match.
    \item ($L2$, $L3$): Topologically equivalent (ignoring already detected patterns).
    \item ($L2$, $L4$): No match.
    \item ($L2$, $L5$): Top toolbar matches the horizontal flow primitive ORC pattern (ignoring already detected patterns). 
    \item After this subsampling step, we have no match pairs: ($L1$, $L3$), ($L1$, $L5$), ($L2$, $L4$), and detected patterns: Left Toolbar: Vertical Flow, Top Toolbar: Horizontal Flow.
    \item Recheck the pair ($L1$, $L3$) and it still has no match, %(ignoring already detected patterns)
    so we subsample ($L1$, $L3$) to get $L6$ (Figure~\ref{fig:example} b). Note: we prefer to first pick the pairs that subsample only a single new exemplar.
    \item ($L1$, $L6$): No match.
    \item ($L3$, $L6$): Topologically equivalent.
    %(ignoring already detected patterns).
    \item After this subsampling step, we have no match pairs: ($L1$, $L5$), ($L2$, $L4$), ($L1$, $L6$), and detected patterns: Left Toolbar: Vertical Flow, Top Toolbar: Horizontal Flow.
    \item Recheck the pair ($L1$, $L6$) and it still has no match, %(ignoring already detected patterns),
    so we subsample ($L1$, $L6$) to get $L7$ (Figure~\ref{fig:example} c).
    \item ($L1$, $L7$): No match.
    \item ($L6$, $L7$): No match.
    \item After this subsampling step, we have no match pairs: ($L1$, $L5$), ($L2$, $L4$), ($L1$, $L7$), ($L6$, $L7$), and detected patterns: Left Toolbar: Vertical Flow, Top Toolbar: Horizontal Flow.
    \item Recheck the pair ($L1$, $L7$) and it still has no match, %(ignoring already detected patterns),
    so we subsample ($L1$, $L7$) to get $L8$ (Figure~\ref{fig:example} d).
    \item ($L1$, $L8$): Detect optional widget 2.
    \item ($L7$, $L8$): Detect optional widget 4.
    \item After this subsampling step, we have no match pairs: ($L1$, $L5$), ($L2$, $L4$), ($L6$, $L7$), and detected patterns: Left Toolbar: Vertical Flow, Top Toolbar: Horizontal Flow, optional widgets 2, 4.
    \item Recheck the pair ($L6$, $L7$) and it still has no match, %(ignoring already detected patterns),
    so we subsample ($L6$, $L7$) to get $L9$ (Figure~\ref{fig:example} e).
    \item ($L6$, $L9$): Detect optional widget 8.
    \item ($L7$, $L9$): Detect optional widget 6.
    \item After this subsampling step, we have no match pairs: ($L1$, $L5$), ($L2$, $L4$), and detected patterns: Left Toolbar: Vertical Flow, Top Toolbar: Horizontal Flow, optional widgets 2, 4, 8, 6.
    \item Recheck the pairs ($L1$, $L5$), ($L2$, $L4$) and they are topologically equivalent. % (ignoring already detected patterns).
    Thus, we do not need to further subsample.
    \item Based on sampled window sizes for optional widgets, the priority/weight of optional widgets: widget 8 > widget 6 > widget 4 > widget 2.
\end{enumerate}

In the end, we have detected the following patterns: Left Toolbar: Vertical Flow, Top Toolbar: Horizontal Flow, and optional widgets 2, 4, 8, 6, with priorities: widget 8 > widget 6 > widget 4 > widget 2.


\subsection{ORC Layout Specification}

We modified ORC layouts~\cite{jiang2019orclayout, jiang2020orcsolver} to provide an API to efficiently define ORC layout specification. For our example, we generate a corresponding ORC layout specification to match the observed layout behaviors and layout patterns:
\begin{equation*}
 \begin{split}
&\textit{HorizontalFlow("HF", topWidgets)}\\
&\textit{VerticalFlow("VF", leftWidgets)}\\
&\textit{widget2.set\_optional()}\\
&\textit{widget4.set\_optional()}\\
&\textit{widget6.set\_optional()}\\
&\textit{widget8.set\_optional()}\\
&\textit{widget2.set\_weight(a)}\\
&\textit{widget4.set\_weight(b)}\\
&\textit{widget6.set\_weight(c)}\\
&\textit{widget8.set\_weight(d)}\\
&\textit{Note:} a < b < c < d.
\end{split}
\end{equation*}
\end{DELETE}



\section{ORC Layout Specification Generation}

In our approach, to identify the layout specification, we apply a grid search to sample layouts with different window sizes and interactively query the interface to extract widget information for each sampled layout size. We then check for topological equivalence between layouts and match sampled layouts with primitive ORC patterns based on the extracted widget information if possible. If we are not successful, we continue to subsample. In the end, we generate a corresponding ORC layout specification.

\subsection{ORC Layout Pattern Matching}

Row change to Column or vice versa 
=> add Pivot before it

sublayout (or widget) X removed, or X suddenly added
=> make X optional

sublayout (or widget) X replaced by Y 
=> Y is alternative for X

X removed from Row and added to (possibly new) adjacent Row
=> merge Rows into HFlow
 


We modified ORC layouts~\cite{jiang2019orclayout, jiang2020orcsolver} to provide an API to efficiently define ORC layout specification. For our example, we generate a corresponding ORC layout specification to match the observed layout behaviors and layout patterns:

\section{Applications}


\subsection{Making Static Layouts Adaptive}

%  \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{figures/application1.png}
% \caption{a) The toolbar of Adobe Photoshop. b) Elements are hidden as the height of the toolbar decreases. c) Elements automatically flow after replacing the original layout with an augmented ORC vertical flow pattern.}
% \label{fig:application1}
% \end{figure}

With the ReverseORC approach, we can turn ordinary, inflexible layouts into more flexible ORC layouts and provide more usability. We can even improve the usability by replacing the original layout with augmented ORC patterns that provide more flexibility in adapting the layout.

For instance, and as a very simple example, the layout of the toolbar of Adobe PhotoShop is static (Figure~\ref{fig:application1} a). When the height of the toolbar is decreased, some elements disappear due to the lack of space (Figure~\ref{fig:application1} b). After we reverse-engineer the panel and replace the original layout with an augmented ORC vertical flow layout pattern, the toolbar elements could reflow adaptively into the toolbar and the width of the toolbar would adjust accordingly (Figure~\ref{fig:application1} c).


\subsection{Creating New GUIs}

%  \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{figures/application2.png}
% \caption{a) The toolbars of GIMP. b) }
% \label{fig:application2}
% \end{figure}

It is often time-consuming for designers to create new GUIs from scratch. Sometimes a designer might find a GUI that matches almost what they are looking for and they then want to create a similar one with minor modifications to the layout. In this case, and instead of manually migrating all the functionality and layout aspects, the ReverseORC method can help designers do such a task quickly and thus accelerate the entire design process. Once we reverse-engineer a GUI and get the corresponding ORC layout specification, it is easy to modify the generated ORC layout specification and use it as a layout template as a base for a variant. Designers can then put new elements into the template (or remove some) to generate a new desired GUI.

For example, GIMP has two separate toolbars (Figure~\ref{fig:application2} a). A designer might want to combine both in a layout shown in Figure~\ref{fig:example}, but without optional widgets. With the ReverseORC approach, we can retrieve the corresponding ORC layout specification for the layout. We then make all widgets non-optional in the ORC layout specification to get a desired layout template. We finally place respective toolbar elements into the template to generate a new GUI so that one toolbar becomes a top toolbar with horizontal flow and the other is a left toolbar with vertical flow (Figure~\ref{fig:application2} b).

\end{DELETE}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX
